Time-to-Green predictions for fully-actuated signal control systems with supervised learning

Recently, efforts have been made to standardize signal phase and timing (SPaT) messages. These messages contain signal phase timings of all signalized intersection approaches. This information can thus be used for efficient motion planning, resulting in more homogeneous traffic flows and uniform speed profiles. Despite efforts to provide robust predictions for semi-actuated signal control systems, predicting signal phase timings for fully-actuated controls remains challenging. This paper proposes a time series prediction framework using aggregated traffic signal and loop detector data. We utilize state-of-the-art machine learning models to predict future signal phases' duration. The performance of a Linear Regression (LR), a Random Forest (RF), and a Long-Short-Term-Memory (LSTM) neural network are assessed against a naive baseline model. Results based on an empirical data set from a fully-actuated signal control system in Zurich, Switzerland, show that machine learning models outperform conventional prediction methods. Furthermore, tree-based decision models such as the RF perform best with an accuracy that meets requirements for practical applications.

==> old_text.tex <==
#############LITERATUR

Should go into the intro of deep learning and why:

Deep learning methods rely on deep neural networks (i.e., with multiple layers). The key difference
between deep learning methods and the traditional machine learning methods is the feature
selection. Deep learning is able to take high dimensional data as input and implicitly select the
feature by training the parameters associated with the complex network architecture, while traditional machine learning methods require manual selection of relevant features. The commonly
used network architectures of deep learning include Multilayer Perceptron (MLP) (e.g.~\cite{ref:habtie}),
Deep Belief Network (DBN) (e.g.,~\cite{ref:huang}), Stacked Auto-Encoder (SAE) (e.g.,~\cite{ref:lv}), Convolutional Neural Network (CNN) (e.g.,~\cite{ref:wang_traffic_speed}), and Recurrent Neural Network (RNN) (e.g.,~\cite{ref:zeng_RNN}),
where MLP, DBN, and SAE are relatively simple networks, CNN has proven to work well for
data with a strong spatial correlation, and RNN is specifically designed to model sequence
data~\cite{ref:wang}. Although our SPaT prediction problem with detector data shares some similarities
with short-term traffic prediction problem, the traffic signal states depend more on the detector
information and can change more frequently. It is still worth investigating how these machine
learning methods can be applied to the SPaT prediction problem.



In our case with rich detector data, it is useful to develop a learning framework to emulate 
the signal control logic by linking the historical SPaT information and sensor 
data (i.e., loop detector and public transport data).

 As the traffic signal is determined solely based on detector
actuation, we expect that there is a strong relationship between the SPaT information and the
detector data.


such as k-nearest neighbor (k-NN)~\cite{ref:chang}, multivariate regression~\cite{ref:sun, ref:clark}, support vector regression (SVR)~\cite{ref:hong, ref:castro_neto, ref:jeong}, random forest~\cite{ref:zhang_RSF}, artificial neural networks (ANN)~\cite{ref:vlahogianni, ref:chan, ref:kumar, ref:tang}, and deep learning methods~\cite{ref:lv, ref:huang, ref:yu_rose, ref:qian}.
%Some of these studies integrate other data sources. For example,~\cite{ref:yu_rose} considered traffic accidents
%data to predict traffic flow in extreme scenarios and~\cite{ref:markou} integrated weather and incident data
%to predict travel demand. 
##################################
ARIMMAAA 

As a first baseline model, the ARIMA model is introduced. ARIMA is a widely used model for forecasting time series. The univariate model can be applied to a stationary time series, which combines auto-regression (by order of $p$) with differencing (by order of $d$) and the moving average method (by order of $q$). Note that here only the historical T2G time series $y_i(t)$ is considered as a model input (i.e., the nonlinear relationship between signal and LD devices is not considered). Consequently, the model is represented by the following equation:
\begin{equation}
    \begin{split}
    \hat{y}'_{i,t} = y_{i,0} + \phi_1 y'_{i,t-1} + ... + \phi_p y'_{i,t-p} +  \\
    \theta_{i,1} \epsilon_{i,t-1} + ... +\theta_{i,p} \epsilon_{i,t-q} + \epsilon_{i,t}.    
    \end{split}
\end{equation}
$ \hat{y}'_{i,t} $ represents the differenced time series denoted as the response variable of signal $i$. The right-hand side of the equation contains the lagged values of $y'_{i,t}$ by the degree of first-order differencing $p$. In addition, the lagged errors $\epsilon_{i,t}$ with the order of the moving average $q$ are included. $\phi_{i,1 ...p}$ and $\theta_{i,1 ...p}$ are parameters. $y_{i,0}$ denotes the intercept. Finally, a suitable model ARIMA($p$, $d$, $q$) is determined for forecasting~\cite{ref:SOWELL_ARIMA}.


##################################### T2G defintion old 
We introduce T2G prediction as a time-series forecast and construct the problem with historical data of signal $i$. $c_i(t)$ denotes the current cycle signal $i$ is operating. $c_i \in \mathcal{C}$ where $\mathcal{C}$ is the set of possible cycles for $i$.

Furthermore, we need to determine the total length of red time of the signal cycle $c_i(t)$, denoted as $r_i(c_i(t))$ and the current time step in a cycle $c$ as $q_i(c_i(t))$. Finally, let $y_i(t)$ be the T2G of a signal $i$ formulated as follows: 
\begin{equation}
     y_i(t) = \left\{
        \begin{array}{ll}
            r_i(c_i(t)) - q_i(c_i(t)), & \quad \text{if $s_i(t) = 0$}   \\
            0, & \quad \text{otherwise.}
        \end{array}
    \right.
    \label{eq:def_3}
\end{equation}
The proposed formulation can be utilized to determine the T2G $y_i(t)$ for a signal $i$ in every cycle $c_i$ when a traffic light is red (i.e, $s_i(t) = 0$). During green ($s_i(t) = 1$), the T2G remains $0$. Consequently, a linear time series is constructed as denoted in (\ref{eq:def_3}). Figure~\ref{fig:time_series} shows $y_i(t)$ for a short time period and a sample traffic signal ($i = 1$) in a morning period; i.e., $y_1(t)$.
\begin{figure}[b]
    \centering
    \includegraphics[width=0.4\textwidth]{images/T2G_Time_Series.pdf}
    \caption{T2G time series for signal device 1; highlighted signal peaks in red correspond to maximum waiting time per cycle.}
    \label{fig:time_series}
\end{figure}




############## block description
The signal peaks in Figure~\ref{fig:time_series} indicate that the maximum of the T2G per cycle (i.e., length of red phase) is not constant and varies between 31 and 66 sec. Note that the latter value might result from approaching public transport that is detected and gets signal priority in the conflicting approach. Hence, the green time of such conflicting approach gets extended, which results in higher waiting times for other streams.

Therefore, these quantities are excluded in the output of Block (1). The outputs are summarized in the set $\mathcal{H}$ and serve as an input to Block (2), where the feature engineering is performed. Here, the most relevant input variables are determined by eliminating correlations and -- if it is a model requirement -- variable transformations are computed. The output of Block (2) is the final feature set $\mathcal{F}$ that functions as an input to Block (3), where the actual training and performance tests are implemented. 

The input is split into training and test data set (70\% and 30\% of the data, respectively). Consequently, a set of models $\mathcal{M}$ is considered, which is specified by the user. After training and testing all elements of $\mathcal{M}$ the best model is selected and predictions for the set of traffic signals are generated. Note that the process of tuning a proper prediction model requires a number of iterations between Block (2) and (3). In this paper, we define an ARIMA, an LR, an RSF and an LSTM model as the members of $\mathcal{M}$. First, the baseline models (i.e., ARIMA and LR) are introduced. Afterwards, we introduce the RSF and LSTM model.



### arima model
ARIMA is a widely used model for forecasting time series. The univariate model can be applied to a stationary time series, which combines auto-regression (by order of $p$) with differencing (by order of $d$) and the moving average method (by order of $q$). Note that here only the historical T2G time series $y_i(t)$ is considered as a model input (i.e., the nonlinear relationship between signal and LD devices is not considered). Consequently, the model is represented by the following equation:
\begin{equation}
    \begin{split}
    \hat{y}'_{i,t} = y_{i,0} + \phi_1 y'_{i,t-1} + ... + \phi_p y'_{i,t-p} +  \\
    \theta_{i,1} \epsilon_{i,t-1} + ... +\theta_{i,p} \epsilon_{i,t-q} + \epsilon_{i,t}.    
    \end{split}
\end{equation}
$ \hat{y}'_{i,t} $ represents the differenced time series denoted as the response variable of signal $i$. The right-hand side of the equation contains the lagged values of $y'_{i,t}$ by the degree of first-order differencing $p$. In addition, the lagged errors $\epsilon_{i,t}$ with the order of the moving average $q$ are included. $\phi_{i,1 ...p}$ and $\theta_{i,1 ...p}$ are parameters. $y_{i,0}$ denotes the intercept. Finally, a suitable model ARIMA($p$, $d$, $q$) is determined for forecasting~\cite{ref:SOWELL_ARIMA}.


##linear regression

where $\hat{y}_{i,o}$ is the T2G (response variable) for signal $i$ and observation $o$, $ \beta_{i,0}$ represents the intercept term and $\beta_{i,1} $ to $\beta_{i,p}$ are the regression coefficients for the $p$ predictors $x_{o,1}$ to $x_{o,p}$ (i.e., the members of the final LD and signal feature set $\mathcal{F}$ described above), respectively. The error term is denoted by $E_{i,o}$ and follows a Gaussian distribution (i.e., $E_{i,o} \sim \mathcal{N}(0, \sigma_{E_{i,o}})$); $T$ denotes the prediction horizon. The solution for $\hat{y}_{i,o}$ is found by applying the Ordinary Least Square (OLS) method. The fitted model can be used to determine a prediction of the T2G for all given traffic signals by obtaining the conditional expected value of the response. To obtain the LR model, the build-in R-package was utilized. Research that similarly introduces LR models within this context can be found in e.g.,~\cite{ref:LR1}.


## pseudo code RSF
To assess the performance of ML models for T2G predictions, two models are introduced. As a first model (and third member of $\mathcal{M}$), an RSF is utilized. The RSF method is based on the concept of survival analysis, i.e., the analysis of time duration until a certain event occurs. Our constructed time series can be analyzed in such a way as it is expected that after the T2G the traffic light switches to green, meaning the time series is 0 for a certain time horizon. Therefore, we utilize the R-package \textit{randomForestSRC}, which implements the pseudo-code presented in Algorithm~\ref{ag:1}, proposed by~\cite{ref:RF}.

For the detailed mathematical background of RSF, the interested reader is referred to~\cite{ref:RF2}.

\begin{algorithm}[t]
\caption{RSF pseudo code}\label{euclid}
\label{ag:1}
\begin{algorithmic}[1]
\Procedure{doRSF}{}
\State 
     \begin{varwidth}[t]{\linewidth}
        $\mathcal{B} \gets$ Bootstrap samples from the original \par
        training data set
        \end{varwidth}

\State 
     \begin{varwidth}[t]{\linewidth}
        $\mathcal{T} \gets$ Grow a survival tree $\forall s \in \mathcal{B}$, \par
        where $s$ is a sample from $\mathcal{B}$
        \end{varwidth}

\State $\mathcal{O} \gets \text{Exclude out-of-bag data from all } s \in \mathcal{B}$
\State 
    \begin{varwidth}[t]{\linewidth}
        Grow tree to full size with the constraint that a leaf \par 
        node $l \in \mathcal{L}$ has no less than $d_0 > 0$ unique \par 
        deaths; $ \mathcal{L}$ is a set of leaf nodes
        \end{varwidth}
\State 
     \begin{varwidth}[t]{\linewidth}
     $\mathcal{C} \gets$ Calculate the Cumulative Hazard Function \par 
     (CHF) $\forall t \in \mathcal{T}$, where $t$ is a survival tree \par 
     for one bootstrap sample 
     \end{varwidth}
\State $\mathcal{P} \gets \text{Calculate prediction error using the set } \mathcal{O}$
\EndProcedure
\end{algorithmic}
\end{algorithm}


##moving window
%\subsection{Moving window procedure}
%\label{sec:window}
%To improve the prediction quality we apply a moving window procedure to the input of the LR and RSF model. Let $w$ be a moving time window in seconds and the matrix $I$ our input matrix which represents all elements of $\mathcal{F}$. The dimension of $I$ is denoted by ${\rm dim}(m_I,n_I)$. To apply our moving window procedure we introduce a transformed matrix $J$ with ${\rm dim}(m_I-w, n_I-w)$. Thereby, the first dimension $m_I-w$ results from the end of the time series as we only consider complete windows. We fill the values of $J$ row by row, each row corresponding the concatenated feature vectors of the corresponding $w$ time steps from $I$. This procedure improves the results significantly as the training process provides inputs at time step $t$ for multiple time instances. Note that according to the model definitions of ARIMA and LSTM a moving window procedure is not applicable. 




###########correlation analysis
As the potential correlation between variables degrades the model quality, we investigate all LDs and signal devices (Figure~\ref{fig:corr_plot}). The data shows almost no correlation between LD devices (except LD 2 and LD3) and between specific LD and signal devices. A more detailed analysis of the signal devices depict some significant positive correlations (e.g., signals 1 and 5 or signals 2 and 6). Nevertheless, this is expected as these signals control compatible traffic streams (see Figure~\ref{fig:intersection}). The same argument holds for the signals regulating pedestrian streams (signal pairs (7,9) and (8, 10)).

The correlation between signals 2 and 3 might occur because the two streams get green at the same time, but the green time for bicycles is smaller as a longer clearing time is required. Consequently, we remove one of the variables that are members of correlated pairs. Note that for this analysis we decide to keep all variables with a correlation coefficient smaller than 0.8. The final signal members of the feature set $\mathcal{F}$ are $i = \{3, 4, 5, 6, 7, 8, 11, 12\}$. For the LDs the devices $j = \{1, 3, 4, 5, 6, 11, 12, 13, 14\}$ are utilized. Consequently, 17 features are used as input LR, RSF, and LSTM models.  
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{images/correlations_shrinked-cropped.pdf}
    \caption{Correlations of all LD (denoted with abbreviation d) and signal devices (denoted with abbreviation sg).}
    \label{fig:corr_plot}
\end{figure}


###data decription
We prove our concept by obtaining a subset of the 15 days' peak hours out of the complete data set. The descriptive statistics of measurements from 7:00am to 10:00am of all days are depicted in Figure~\ref{fig:hists}.



###result table

\begin{table*}[t]
\centering
\caption{Model performance comparison on the test data set with the $\overline{\rm MAE}$, $\overline{\rm RMSE}$ and corresponding $\sigma_{\text{MAE}}$, $\sigma_{\text{RMSE}}$ respectively for ARIMA, LR, RSF and LSTM.}
\resizebox{2.0\columnwidth}{!}{%
\begin{tabular}{{R{0.3cm}R{0.64cm}R{0.64cm}R{0.78cm}R{0.64cm}|R{0.64cm}R{0.64cm}R{0.78cm}R{0.64cm}|R{0.64cm}R{0.64cm}R{0.78cm}R{0.64cm}|R{0.7cm}R{0.7cm}R{0.78cm}R{0.64cm}R{0.64cm}R{0.64cm}R{0.64cm}R{0.64cm}}}
\toprule
 & \multicolumn{4}{c}{ARIMA} & \multicolumn{4}{c}{LR} & \multicolumn{4}{c}{RSF} &  \multicolumn{4}{c}{LSTM} \\
 $i$        & $\overline{\rm MAE}$          & $\sigma_{\text{MAE}}$      & $\overline{\rm RMSE}$          & $\sigma_{\text{RMSE}}$     & $\overline{\rm MAE}$        & $\sigma_{\text{MAE}}$   & $\overline{\rm RMSE}$          & $\sigma_{\text{RMSE}}$       & $\overline{\rm MAE}$         & $\sigma_{\text{MAE}}$   &  $\overline{\rm RMSE}$          & $\sigma_{\text{RMSE}}$        & $\overline{\rm MAE}$  & $\sigma_{\rm{MAE}}$  & $\overline{\rm RMSE}$  & $\sigma_{\text{RMSE}}$  \\
\midrule
1 & 17.09 & 4.03    & 19.93 &  4.72   & 2.53      & 0.73  & 4.37  &   1.45   & 1.24   & 0.51   & 3.01     & 1.29  & 0.39  &  0.06 & 0.41  & 0.05 \\
2 & 18.52 & 2.62    & 22.12 &  3.05   & 2.32      & 0.60  & 3.63  &   0.93   & 1.15   & 0.41   & 2.44     & 0.89  & 0.37  & 0.02  & 0.40  & 0.02 \\
3 & 18.42 & 2.65    & 21.71 &  3.06   & 2.30      & 0.78  & 3.62  &   1.31   & 1.12   & 0.63   & 2.44     & 1.35  & 0.34  &  0.03 & 0.38  & 0.03 \\
4 & 17.55 & 4.20    & 20.52 &  4.95   & 2.65      & 0.78  & 4.45  &   1.54   & 1.15   & 0.54   & 2.76     & 1.48  & 0.34  & 0.02  & 0.39  & 0.02 \\
5 & 17.36 & 4.61    & 20.44 &  5.33   & 2.32      & 0.74  & 4.05  &   1.69   & 1.31   & 0.59   & 3.05     & 1.70  & 0.33  & 0.02  & 0.38  & 0.02 \\
6 & 18.26 & 2.66    & 21.95 &  3.12   & 2.54      & 0.65  & 4.03  &   1.00   & 1.13   & 0.35   & 2.41     & 0.82  & 0.38  & 0.02  & 0.41  & 0.02 \\
7 & 13.63 & 2.15    & 17.58 &  2.34   & 2.13      & 0.60  & 3.49  &   0.96   & 0.64   & 0.29   & 1.53     & 0.89  & 0.28  & 0.02  & 0.35  & 0.02 \\
8 & 11.64 & 4.53    & 15.23 &  5.52   & 2.60      & 0.73  & 4.45  &   1.52   & 1.37   & 0.57   & 3.40     & 1.46  & 0.25  & 0.02  & 0.33  & 0.01 \\
9 & 14.58 & 1.12    & 16.99 &  1.30   & 2.17      & 0.25  & 3.97  &   0.39   & 1.17   & 0.28   & 3.50     & 0.51  & 0.26  & 0.03  & 0.34  & 0.02 \\
10& 12.26 & 5.89    &14.30  & 6.80    & 2.66     & 1.09  & 4.81  &   1.93   & 1.24   & 0.65   & 3.46     & 1.68  & 0.22  & 0.03  & 0.31  & 0.02 \\
11&  86.58 & 19.08  & 112.46 &  24.74 & 74.51     & 11.95 & 92.96 &  16.83   & 69.02  & 12.05  & 92.82    & 16.06 & 0.42  & 0.03  & 0.43  & 0.02 \\
12& 95.18  & 47.92 & 119.77 &  59.22   & 91.11     & 30.44 & 111.16&  40.28   & 82.06  & 30.40  & 108.10   & 37.97 & 0.39  & 0.06  & 0.41  & 0.05 \\
\bottomrule
\end{tabular}
}
\label{tab:results}
\end{table*}


#### result description LR
The LR model is applied with standard settings and no variable transformations. Nevertheless, the general assumptions required to justify the application of OLS are considered in the analysis. A window size of $w=10$ is chosen. 
The model shows that $92$ out of $170$ parameters are statistically significant on the 95\% level and the adjusted $R^2$ is determined to $0.89$.


#### old RF explanation
The RSF is applied with a number of trees $n = 100$; $n$ is chosen considering the trade-off between gain in improvement versus the increase in computational time. Furthermore, the data is centered and scaled to obtain better model performance. Again, the window size is chosen with $w=10$. Analyzing the model output shows that the RSF model explains $95.62\%$ of the training data's variance with an average number of terminal nodes of $11951.28$. The LSTM model was trained with 50 epochs and a batch size of 2000. The architecture is specified with 50 hidden layers and the first layer is designed according to the shape of the input data. To ensure a valid model quality, the loss function ($\rm MAE$) was analyzed to prevent the model from overfitting the training data. 
To allow a performance comparison between the models, we test all members of $\mathcal{M}$ on the test data set and show the $\overline{\rm MAE}$ for all calculated errors and the corresponding standard deviation $\sigma_{\text{MAE}}$ in Table~\ref{tab:results}.


###old plots and results description

The results show that a simple ARIMA model is not a promising approach for T2G predictions. $\overline{\rm MAE}$ values with the corresponding variances $\sigma_{\rm MAE}$ exceed substantially the accuracy requirements for application (values between 11.64 sec and 95.18 sec, with a corresponding high $\sigma_{\rm MAE}$). The result underlines the hypotheses that simple forecasting models considering only the T2G time series are not suitable for our prediction problems. Furthermore, Figure~\ref{fig:perf_arima} shows a prediction sample from 10:50am to 11:00am of the test data set. The ARIMA model does not capture the pattern of a T2G time series, which results in high under- or over-estimation of the residual times. The model provides an estimate for the next phase, but the signal remains constant afterwards. Hence, ARIMA can only be used to predict the next phase and gives predictions of unsatisfactory accuracy.
\begin{figure}[!b]
    \centering
    \includegraphics[width=0.4\textwidth]{images/comp_test_arima.pdf}
    \caption{Prediction sample from the test data set of the T2G for a 10 minutes time frame with the ARIMA model.}
    \label{fig:perf_arima}
\end{figure}

The LR model provides $\overline{\rm MAE}$ values between 2.13 and 2.66 sec for traffic lights that regulate vehicle traffic streams (signals 1 to 10). For public transport signals, the prediction accuracy shows a high error. This is because the model is not able to capture the signal peaks that occur when there is no demand on these streams. An example of this behavior is depicted in Figure~\ref{fig:perf_lm} (signal peak at 11:00am). Besides, the linear model suffers from negative values during the period that T2G is zero and is also likely to miss such signal patterns, which result in a constant T2G greater than zero (Figure~\ref{fig:perf_rsf} 11:02am). 
\begin{figure}[!b]
    \centering
    \includegraphics[width=0.4\textwidth]{images/comp_test_lm.pdf}
    \caption{Prediction sample from the test data set of the T2G for a 10 minutes time frame with the LR model.}
    \label{fig:perf_lm}
\end{figure}

The RSF model demonstrates the second best performance with $\overline{\rm MAE}$ ranging from 0.64 to 1.37 sec for signals 1--10, with a corresponding low variance $\sigma_{\rm MAE}$. For signal 11 and signal 12, the model also fails to capture high signal peaks accurately. Nevertheless, the RSF prediction never misses a green phase (when T2G is zero). A sample prediction is shown in Figure~\ref{fig:perf_rsf} with the described behavior.
\begin{figure}[!b]
    \centering
    \includegraphics[width=0.4\textwidth]{images/comp_test_rsf.pdf}
    \caption{Prediction sample from the test data set of the T2G for a 10 minutes time frame with the RSF model.}
    \label{fig:perf_rsf}
\end{figure}
Our best candidate is the LSTM neural network where the condition $\overline{MAE} < 1$ holds for all signals. The highest error value can be depicted for signal 11 with an $\overline{MAE}$ of 0.42 and $\sigma_{\rm MAE}$ of 0.03. This corresponds to an $\overline{RMSE}$ of 0.43 with $\sigma_{\rm MAE}$ of 0.02.  Figure~\ref{fig:perf_lstm} shows the test and prediction data with an accurate fit of the time series. 
\begin{figure}[!b]
    \centering
    \includegraphics[width=0.4\textwidth]{images/comp_test_lstm.pdf}
    \caption{Prediction sample from the test data set of the T2G for a 10 minutes time frame with the LSTM model.}
    \label{fig:perf_lstm}
\end{figure}
Therefore, an LSTM should be utilized as a generic and flexible tool for predicting the T2G series of a traffic signal. Compared to the RSF the error values decrease significantly and the model is able to capture more irregular patterns for traffic lights of public transport. In addition, the LSTM meets the accuracy requirement for T2G predictions.

Finally, we utilize our two best candidates (RSF and LSTM) and test the trained models in a peak-hour scenario of another weekday. We determine $10$ minutes of historical data and test the prediction performance on the following $10$ minutes. Figure~\ref{fig:another_test_rsf} depicts the prediction with the RSF model.
\begin{figure}[!b]
    \centering
    \includegraphics[width=0.4\textwidth]{images/comp_test_another_day_rsf.pdf}
    \caption{Prediction of 10 minutes T2G in the peak-hour of another weekday with the RSF model.}
    \label{fig:another_test_rsf}
\end{figure}
It can be shown that in general the prediction is within the accuracy requirements but fails to predict the last T2G peak. A test of the LSTM model on the 10 minute time frame shows an accurate forecast and no miss of a signal peak is detected. As depicted in Figure~\ref{fig:another_test_lstm} the T2G prediction are within the accurancy requirements and can be applied to real-world applications. 
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.4\textwidth]{images/comp_test_another_day_lstm.pdf}
    \caption{Prediction of 10 minutes T2G in the peak-hour of another weekday with the LSTM model.}
    \label{fig:another_test_lstm}
\end{figure}



Last we propose the RFDS methodology which incorporates the RF introduced above. However, the RFDS constitutes a pipeline where three RF models are trained on subsets of the training data. This methodology allows to tackle long-tailed feature and/or target distributions. E.g., a high red time of traffic signal can reflect high traffic demand or public transportation priority for a conflicting traffic stream. Consequently, a long-tailed data distribution is given, where the input samples can not be treated as outliers and eliminated. 

The subsets are calculated by utilizing a lower and upper percentile threshold, $\mathrm{PC}_a$ and $\mathrm{PC}_b$, respectively. By deriving three subsets of training data sets, the resulting models (low, middle, and high) are trained and evaluated only on the corresponding subsets. The models are then integrated into the pipline depicted in Figure~\ref{fig:rfds}. A decision block evaluates a new input sample $X$ based on the percentile $\mathrm{PC}_i$. $\mathrm{PC}_i$ calculates based on the input feature representing the red time of signal $i$ of $X$; i.e., $X[r_i(c_{i,n})]$. This is valid as the T2G target is the red time of the next occuring cycle. Consequently, the distribution of the input feature and the target are identical. Dependent on the result of $\mathrm{PC}_i$ the model selection is performed and the prediction of $\hat{Y}_i(c_{i,n})$ computed. Note that the percentile thresholds $\mathrm{PC}_a$ and $\mathrm{PC}_b$ are treated as hyperparameters. As the performance of the final RFDS method is also dependent on the percentile thresholds it is crucial to include both parameters into the hyperparameter tuning procedure.   

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/RFDS_framework.pdf}
    \caption{Random forest with distribution split, where the model selection is based on the input percentile $\mathrm{PC}_i$. $\mathrm{PC}_a$ and $\mathrm{PC}_b$ denote the lower and upper percentile, respectively.}
    \label{fig:rfds}
\end{figure}


We then implement a methodology for handling long-tailed distributed input features and target variables. The framework allows to find the best distribution split based on percentiles, train separate models based on the separation, and utilize the corresponding model based on the given input sample.



 %On the other hand, there could be a delay between the activation of a detector and the change in the signal state. Therefore, it is also important to consider the temporal relation between the traffic signals and the detectors as well.
 
 
 
 %Utilizing the signal states of all available traffic lights and LDs, a feature set for every traffic light's cycle $c_{i,n}$ can be computed. Note that fully-actuated systems allow for diverging cycle lengths $c$ fo


%The objective of this work is to predict the next T2G based on utilizing traffic signal and detector data of an urban intersection.

%Aiming for the prediction of the T2G $\hat{Y}_{i}(c_{i,n})$ of traffic light $i$, one needs to consider that fully-actuated signal control systems allow for non-constant red, green, and cycle times. Consequently, the T2G target is dependent on the cycle $c$ of a traffic light $i$ and the index of the present cycle as a prediction input; i.e., $c_{i,n}$. The problem is then formulated as $\hat{Y}_{i}(c_{i,n}) = f(\textbf{X})$. The function $f(\textbf{X})$ denotes the relationship between the set of input features $\textbf{X}$ and the target $\hat{Y}_{i}(c_{i,n})$. Note that the T2G prediction corresponds to the red time of the next cycle $c_{i,n+1}$. 

%This statement is supported by the prediction results for the traffic lights utilized for public transportation (11, 12): the error values (MAE and RMSE) are significantly higher than the presented results. This is due to a higher variance of the T2G time series (e.g., a very long red phase due to no tram arrival followed by a short red phase when two trams are arriving). The MAE/RMSE of signals 11 and 12 are 220.23/248.19 sec and 212.05/240.27 sec, respectively. Note here that a prediction model that just utilizes the average red time of a historical data set would show already a better performance. Also, the EH and NM ratio is below 1\%, respectively. 
